VidHarm: A Clip Based Dataset for Harmful Content Detection

Automatically identifying harmful content in video is an important task with a wide range of applications. However, there is a lack of professionally labeled open datasets available. In this work VidHarm, an open dataset of 3589 video clips from film trailers annotated by professionals, is presented. An analysis of the dataset is performed, revealing among other things the relation between clip and trailer level annotations. Audiovisual models are trained on the dataset and an in-depth study of modeling choices conducted. The results show that performance is greatly improved by combining the visual and audio modality, pre-training on large-scale video recognition datasets, and class balanced sampling. Lastly, biases of the trained models are investigated using discrimination probing. VidHarm is openly available, and further details are available at: https://vidharm.github.io

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> analysis.tex <==
From our quantitative results and qualitative examples, it is clear that our models can understand complex forms of harmful content when trained on our dataset. However, as our failure cases indicate, a true general understanding is not quite achieved. As is indicated by our failure case in Example 4, our visual model sometimes misjudges threatening contexts. This is not surprising, as determining the harmfulness of context is a difficult task even for humans. Our audio model faces issues related to language understanding, sometimes missing threatening language. Since our dataset is multilingual, a general understanding would require an audio model capable of multilingual speech recognition and advanced language understanding, which we consider unlikely to emerge from our relatively small networks and dataset. 

It is furthermore clear that both modalities must be utilized for a true understanding. While the visual and audio modalities achieves similar performance in expectation, they can perform vastly differently for the individual clips. We believe this is directly related to the task. Many scenes contain harmful information only in a single modality, which is shown in our qualitative examples. Hence an obvious conclusion is that the interaction between audio and video is vital for truly understanding harmful content. Yet, from our experiments we found the highest performance was achieved by a very simple model of interaction. Difficulties in training multimodal models have been observed in several recent works \cite{wang2020makes,Xiao2020}, where it is argued that special care must be taken to combat overfitting.

==> futurework.tex <==
%In many real-world applications, it is interesting to have a single prediction for much longer sequences,  e.g., an entire movie. Extending the dataset and training models on long sequences comes with great challenges, such as retaining computational tractability.

The proposed dataset is currently limited to movie trailers from a limited set of distributors. A greater selection of distributors may give a greater diversity in types of content.
%Another important topic is that of fairness and equality. Biases and skewness may occur in all stages of the machine learning process. In this work gender bias was investigated, and found to exist in some trained models. As future work, preventing models from learning unwanted biases~\cite{silberg2019notes}, e.g. by adversarial learning~\cite{zhang2018mitigating}, will be further investigated.

%Finally, incorporating more advanced multi-modal models may improve performance. However, difficulties in training multimodal models have been observed in several recent works \cite{wang2020makes,Xiao2020}, where it is argued that special care must be taken to combat overfitting.

==> rebuttal.tex <==
We are thankful to all reviewers for their comments and feedback. While the reviewers agreed that our dataset is important and novel, they also had some suggestions and concerns. In particular we appreciate the suggestions regarding making the novelty and statistics of our dataset compared to previous datasets more clear. In this version we have made substantial improvements in the paper regarding those aspects, as well as other improvements suggested by the reviewers. 


We now address the individual comments and suggestions from the reviewers.

\subsection*{Reviewer 1}
We thank the reviewer for the comments and suggestions.

Suggestions from the reviewer:
\begin{enumerate}
    \item \textit{Add more in-depth descriptions on the advantages of the
dataset VidHarm over other datasets, e.g. providing
different scale of datasets, visualization of comparison
graphs}

We agree that the benefits of the proposed dataset was not discussed clearly enough in the initial version.
To address this, we provide additional details about the diversity of data compared to previous proposed datasets and the importance of professional labels (Table \ref{tab:datasets}, and section \ref{sec:dataset_relevance}).%  \textcolor{red}{You should also say where in the paper you have added these details}

\item \textit{Add and implementing SOTA methods from previous work on
this dataset and other datasets for comparison?}

Both our video and audio recognition models are strong baselines which have  achieved SOTA results on related datasets such as Kinetics. While we agree that further comparisons are of interest, our main focus in this paper is not benchmarking of all SOTA models, but rather establishing a solid baseline and to gain a deeper understanding of the proposed dataset. For that reason, we do not add additional models to the evaluation, however, in future work a review paper including benchmarking of available SOTA approaches is of interest.

\item \textit{Add more in-depth work on qualitative and quantitative
experiments?}

We include two additional metrics mean Precision / mean Recall (eq. \ref{eq:mp}, \ref{eq:mr}), to compare against the proposed evaluation metric. We found, among other things, that while learned fusion models may increase mR and mP, they do not necessarily increase CAE (Section \ref{sec:late_fusion_resuls}).
\end{enumerate}

\subsection*{Reviewer 2}
We thank the reviewer for the comments and suggestions.
\begin{enumerate}
    \item \textit{The proposed annotated dataset is very important for the
research community and is very challenging ensure the
quality. The dataset should be made open available so that
reviewers can assess the contribution.}

We are happy to hear that the reviewer considers the dataset as very important. We additionally agree with the reviewer that open access is important. In the initial version, a link to the dataset webpage was given in the abstract, from where the dataset was openly available to download. In this version we further clarify this, and additionally make the code for model evaluation openly available, the link to which is posted in the dataset webpage. We reiterate that the \textbf{dataset is openly available}.

\item \textit{These clips are given hash names and are then given in
random order to two professional film classifiers, i.e.,
each clip is labeled by two people. For all clips where the
classifiers disagree, a second review is conducted jointly
and a refined label produced.” The authors are suggested to
describe the level and background of the annotators in
detail.}

We agree with the reviewer that this is important, given our emphasis on professionally curated labels. In this version we provide further details on the annotators (Section \ref{sec:data_acquisition}).

\item \textit{Sufficient comparative experiments are lacking to prove
the advantage of the proposed method. The authors are
suggested to undertake more experiments.}

We would like to emphasize that the main focus of our paper is the proposed dataset, and accompanying analysis. However, we agree that the experimental evaluation was lacking in the first version, and have therefore added two additional metrics. See Reviewer 1, suggestion 3.
\end{enumerate}
\subsection*{Reviewer 3}
We thank the reviewer for considering our work well organized and easy to understand. We address comments and suggestions below.  

\begin{enumerate}
    \item \textit{Statistics of the dataset are missing, especially
statistics of the rating categories.
}
We agree with the reviewer that rating category statistics are important, and have therefore added them in this version (Fig. \ref{fig:classdistribution}). Additionally, we have added statistics regarding the number of different languages. (Table \ref{tab:datasets} and Section \ref{sec:data_description}).
\item \textit{Adding a general plot of the architecture is suggested.}
We agree that this would be beneficial. However, due to lack of space and our focus being mainly on the dataset, we refer to the works of \cite{He2016} and \cite{Feichtenhofer2019} for further details.

\item \textit{One metric is usually not enough for evaluating the
model on the dataset. For example, the proposed CAE could
evaluate the precision of the model well. But the
evaluation of recall is missing.}

We agree with the reviewer that the initial paper was lacking in comparative metrics. Our improvements in this version is described in Reviewer 1, suggestion 3.

\item \textit{In addition, I am interested in whether the dataset would
provide the caption/ASR caption for each video.
}

We do not currently provide such captions in part due to the fact that our dataset contains at least 37 distinct languages, however since audio files are available, automatic captioning is possible. Additionally since the trailers are publicly released movies, there might also be possibilities of gathering subtitles from official sources or from crowd-sourcing.
 	
\end{enumerate}

